Beyond Losses Reweighting: Empowering Multi-Task Learning via the Generalization Perspective

Multi-task learning (MTL) trains deep neural networks to optimize several objectives simultaneously using a shared backbone, which leads to reduced computational costs, improved data efficiency, and enhanced performance through cross-task knowledge sharing. Although recent gradient manipulation techniques aim to find a common descent direction that benefits all tasks, conventional empirical loss minimization still leaves models vulnerable to overfitting and gradient conflicts. To address this, we introduce a novel MTL framework that leverages weight perturbation to regulate gradient norms, thus improving generalization. By adaptively modulating weight perturbations, our approach harmonizes task-specific gradients, reducing conflicts and encouraging more robust learning across tasks. Theoretical insights reveal that controlling the gradient norm through weight perturbation directly contributes to better generalization. Extensive experiments across diverse applications demonstrate that our method significantly outperforms existing gradient-based MTL techniques in terms of task performance and overall model robustness.

==> sec/3_background.tex <==
\section{Background}
\label{sec:backgroun}

% In this section, we formally introduce the notions of multi-objective optimization and reformulate the general setting for multi-task learning. We then recap the training of sharpness aware minimization .

% \subsection{Multi-objective optimization}
% Assume that we are given $m$ objectives functions $\mathcal{L}^{i}(\boldsymbol{\theta})$, $i\in[m]$
% where $\boldsymbol{\theta}\in\ensuremath{\mathbb{R}^{d}}$, each $\mathcal{L}^{i}:\ensuremath{\mathbb{R}^{d}}\ensuremath{\rightarrow\mathbb{R}}$ is a scalar-valued function,  and we denote $[m]:= \{1,2,\dots,m\}$. 

% In the multi-objective optimization (MOO) problem, we are interested in minimizing a vector-valued objective function $\boldsymbol{\mathcal{L}}(\boldsymbol{\theta})$ defined as:
% \begin{equation}
% \boldsymbol{\mathcal{L}}(\boldsymbol{\theta})=[\mathcal{L}^{1}(\boldsymbol{\theta}),\mathcal{L}^{2}(\boldsymbol{\theta}),\dots,\mathcal{L}^{m}(\boldsymbol{\theta})].\label{eq:moo}
% \end{equation}

% Given two feasible solutions $\boldsymbol{\theta}$ and $\boldsymbol{\theta}'$, we say that $\boldsymbol{\theta}$ dominates $\boldsymbol{\theta}'$ (i.e., $\boldsymbol{\theta} \prec \boldsymbol{\theta}'$) if and only if $\mathcal{L}^{i}(\boldsymbol{\theta})\leq \mathcal{L}^{i}(\boldsymbol{\theta}')$ $ \forall i \in [m]$
% and $\exists$ $j\in[m]$ s.t. $\mathcal{L}^{j}(\boldsymbol{\theta})<\mathcal{L}^{j}(\boldsymbol{\theta}')$.

% By the above definition of \textbf{Pareto dominance}, we can compare two given feasible solutions $\boldsymbol{\theta}$ and $\boldsymbol{\theta}'$, which leads us to the definition of Pareto optimality.   

% \noindent
% \textbf{Pareto optimality.} A solution $\boldsymbol{\theta}^{*}$ in the optimization problem
% (\ref{eq:moo}) is said to be a local Pareto optimality if it is not dominated
% by any other solution in its vicinity. 
% Therefore, the solution set of the MOO problem is given by $\mathcal{P}:=\left\{ \boldsymbol{\theta}^{*}\mid\nexists \boldsymbol{\theta}^{\prime}:\boldsymbol{\theta}^{\prime} \prec \boldsymbol{\theta}^{*}\right\} $.
% This set of all Pareto optimal solutions is called the Pareto set,
% while the collection of their images in the objective space is called the Pareto front.


% In general, an optimal solution for this objective vector function
% does not exist since each of the individual function $\mathcal{L}^{i}(\boldsymbol{\theta})$ does
% not necessarily guarantee to have the same minimum solution. Alternatively,
% we expect to obtain a solution, from which we cannot improve any specific
% objective without hurting another (i.e. a Pareto stationary solution).
% According to the above formulation, the solution \citep{zitzler1999multiobjective}
% of the multi-objective minimization problem is formally defined as
% follows:

% \textbf{Pareto dominance} Let $\boldsymbol{\theta}_{1},\boldsymbol{\theta}_{2}$ be two solutions for
% the multi-objective optimization problem in Equation \ref{eq:moo},
% $\boldsymbol{\theta}_{1}$ dominates $\boldsymbol{\theta}_{2}$ $(\boldsymbol{\theta}_{1} \prec \boldsymbol{\theta}_{2})$ if and only if $\mathcal{L}^{i}(\boldsymbol{\theta}_{1})\leq \mathcal{L}^{i}(\boldsymbol{\theta}_{2})$ $ \forall i \in [m]$
% and $\exists$ $j\in[m]$ s.t. $\mathcal{L}^{j}(\boldsymbol{\theta}_{1})<\mathcal{L}^{j}(\boldsymbol{\theta}_{2})$.


% \subsection{Multi-task learning}
% Multi-task learning (MTL) can be viewed as a specific application of MOO. For MTL, we assume a data-label distribution $\mathcal{D}$ from which we can sample a training set $\mathcal{S}= \{(\boldsymbol{x}_i,y_i^1,...,y_i^m)_{i=1}^n\}$, where $\boldsymbol{x}_i$ is a data example and $y_i^1,...,y_i^m$ are the labels of the tasks $1,2,...,m$ respectively. 

% The model for each task $\boldsymbol{\theta}^i = [\boldsymbol{\theta}_{sh}, \boldsymbol{\theta}^i_{ns}]$ consists of the shared part $\boldsymbol{\theta}_{sh}$ and the individual non-shared part $\boldsymbol{\theta}^i_{ns}$. We denote the general loss for task $i$ as $\mathcal{L}^i_{\mathcal{D}}(\boldsymbol{\theta}^i)$, while its empirical loss over the training set $\mathcal{S}$ as $\mathcal{L}^i_{\mathcal{S}}(\boldsymbol{\theta}^i)$.
% Existing works in MTL, typically MGDA \citep{sener2018multi}, PCGrad \citep{yu2020gradient}, CAGrad \citep{liu2021conflict}, and IMTL \citep{liu2021towards} aim to find a model that simultaneously minimizes the empirical losses for all tasks:
% \begin{equation}
%     \min_{\boldsymbol{\theta}_{sh},\boldsymbol{\theta}_{ns}^{1:m}}\left[\mathcal{L}_{\mathcal{S}}^{1}\left(\boldsymbol{\theta}^{1}\right),...,\mathcal{L}_{\mathcal{S}}^{m}\left(\boldsymbol{\theta}^{m}\right)\right].
% \end{equation}

% However, these works only focus on minimizing the empirical losses and does not concern the general losses which assist the model in combating overfitting. In this work, analogous to SAM \citep{foret2021sharpnessaware}, we develop upper bounds for the task general losses in the context of MTL and then rely on these upper bounds to devise a novel MTL framework via seeking the task-based flat regions.   

% Consider a general multi-task learning setting, where we are given a fixed-capacity model parameterized by $\boldsymbol{\theta}$ and $m\geq 2$ correlated tasks, each of which is characterized by a loss function  $\mathcal{L}^i \in \{\mathcal{L}^1, \mathcal{L}^2, \dots, \mathcal{L}^m\}$.  In the MTL learning scenario, we aim to find the optimal $\boldsymbol{\theta}^*$ such that our model that can perform well across tasks simultaneously.
% Note that the model parameter $\boldsymbol{\theta}$ is often composed of two parts: $\boldsymbol{\theta}_{sh}$ as the feature extractor that is shared among tasks, and a list of $\{\boldsymbol{\theta}_{ns}^i\}_{i=1}^m$ each of which is specified for each task. 

% Generally, in a multi-task learning setting, all the tasks share one common dataset. Suppose a training dataset $\mathcal{S}$ that independently and identically follows an underlying distribution $\mathcal{D}$, the optimal parameter can be approximated by minimizing the average empirical loss over all tasks: $\boldsymbol{\theta^*} = \arg \min_{\boldsymbol{\theta}} \frac{1}{m} \sum_{i=1}^m \mathcal{L}^{i}_S(\boldsymbol{\theta})$. The empirical loss function for task $i^{\text{th}}$ is, for example in the supervised setting, defined as $\mathcal{L}^{i}_S(\boldsymbol{\theta}) = \frac{1}{|\mathcal{S}|}\sum_{i=1}^{|\mathcal{S}|} \mathcal{L}^{i} (\boldsymbol{\theta}, \boldsymbol{\theta}_i, y_i)$, where $ \mathcal{L}^{m} (\boldsymbol{\theta}, \boldsymbol{\theta}_i, y_i)$ is the per-data-point loss function. Similarly, the population loss for task $m$ is $\mathcal{L}^{i}_D(\boldsymbol{\theta}) = \mathbb{E}_{(x,y) \sim D} \bigr[\mathcal{L}^{i} (\boldsymbol{\theta}, x, y) \bigr]$. 

%\section{Sharpness aware minimization training}
Conventional methods that focus on minimizing the empirical loss can be easily prone to overfitting problems (i.e., the validation error no longer decreases, but the training loss keeps declining), thus, restricting model generalization performance. In an attempt to alleviate such phenomenons, ~\citep{foret2021sharpnessaware, zheng2021regularizing, wu2020adversarial} proposed to find minima whose neighbors also having low loss values, which can be done by optimizing the following worst-case perturbation loss
\begin{align}
    \underset{\boldsymbol{\theta}}{\min} \underset{||\boldsymbol{\epsilon}||_2 \leq \rho}{\max} \mathcal{L}\left({\boldsymbol{\theta}+\boldsymbol{\epsilon}}\right), \label{eq:sharp_minimization}
\end{align} where $||\cdot||_2$ denotes the $l_2$ norm and $\rho$ represents the radius of the neighborhood.  

To solve problem~\eqref{eq:sharp_minimization}, ~\citep{foret2021sharpnessaware} proposed to first find the solution for the inner maximization by approximating $\mathcal{L}(\boldsymbol{\theta}+\boldsymbol{\epsilon})$ via a first-order Taylor expansion w.r.t $\boldsymbol{\epsilon}$ around $0$, which is as follows:
% {\small
\begin{align*}
    \boldsymbol{\epsilon}^* =\underset{||\boldsymbol{\epsilon}||_2 \leq \rho}{\arg \max} \ \mathcal{L} (\boldsymbol{\theta}+\boldsymbol{\epsilon}) 
    %&
    \approx \mathop{\arg \max}\limits_{||\boldsymbol{\epsilon}||_2 \leq \rho} \ \boldsymbol{\epsilon}^{\top}  \nabla_{\boldsymbol{\theta}}\mathcal{L}(\boldsymbol{\theta}) %\\ 
    %&
    \approx \rho\frac{\nabla_{\boldsymbol{\theta}}\mathcal{L}(\boldsymbol{\theta})}{||\nabla_{\boldsymbol{\theta}}\mathcal{L}(\boldsymbol{\theta})||_2}.
\end{align*}
% }
Putting into words, the worst-case perturbation is approximated as the scaled gradient of the loss w.r.t. the current parameter $\boldsymbol{\theta}$. Then, the gradient w.r.t this perturbed model is computed to update $\boldsymbol{\theta}$:
\begin{equation}
    \boldsymbol{g}^{\text{SAM}} :=\nabla_{\boldsymbol{\theta}} \underset{||\boldsymbol{\epsilon}||_2 \leq \rho}{\max} \mathcal{L}\left({\boldsymbol{\theta}+\boldsymbol{\epsilon}}\right) \approx \nabla_{\boldsymbol{\theta}} \mathcal{L}(\boldsymbol{\theta}+\boldsymbol{\epsilon})|_{\boldsymbol{\theta}+\boldsymbol{\epsilon}^*}
    \label{eq:sam_grad}
\end{equation}
